Deep Music Information Dynamics

Music comprises of a set of complex simultaneous events organized in time. In this paper we introduce a novel framework that we call Deep Musical Information Dynamics, which combines two parallel streams - a low rate latent representation stream that is assumed to capture the dynamics of a thought process contrasted with a higher rate information dynamics derived from the musical data itself. Motivated by rate-distortion theories of human cognition we propose a framework for exploring possible relations between imaginary anticipations existing in the listener's mind and information dynamics of the musical surface itself. This model is demonstrated for the case of symbolic (MIDI) data, as accounting for acoustic surface would require many more layers to capture instrument properties and performance expressive inflections. The mathematical framework is based on variational encoding that first establishes a high rate representation of the musical observations, which is then reduced using a bit-allocation method into a parallel low rate data stream. The combined loss considered here includes both the information rate in terms of time evolution for each stream, and the fidelity of encoding measured in terms of mutual information between the high and low rate representations. In the simulations presented in the paper we are able to juxtapose aspects of latent/imaginary surprisal versus surprisal of the music surface in a manner that is quantifiable and computationally tractable. The set of computational tools is discussed in the paper, suggesting that a trade off between compression and prediction are an important factor in the analysis and design of time-based music generative models.

==> paper_contents_long.tex <==
\section{Introduction}
Music Information Dynamics is a field in music analysis that is inspired by theories of musical anticipation \cite{meyer56emotion}\cite{huron06sweet}, which deals with quantifying the amount of information passing over time between past and future in musical signal \cite{dubnov06spectral},\cite{Abdallah}. Music Information Dynamics can be estimated in terms of Information Rate, which is defined as mutual information between past and future of a musical signal. Generative models that maximize Information rate were shown to provide good results in machine improvisation systems %cite{Assayag2004},
\cite{pasquier2017introduction}. Since music is constantly changing, the ability to capture structure in time depends on the way similarity is computed over time
%a sequence of representation vectors. 
For example, two musical measures improvised on same sequence of chords often have different notes because of voicing considerations, rhythms changes, embellishments and more. Accordingly, finding repetitions in time require representations that are robust to statistical variations in the signal. In this paper we introduce the concept of deep musical information dynamics analysis that offers a combined approach to learning representation and predictive information, considering the trade off between encoding complexity of short-term musical structures and maximizing the information rate from past into future. 

%------

\section{Deep Information Dynamics}
The underlying motivation in proposing a deep information model is to acknowledge the fact that imagination, both for the composer, improviser and the listener, is playing an important and possibly even a crucial role in experiencing and creation of music. Music generation and listening are active processes that involve simultaneous processing of the incoming musical information in order to extract salient features, while at the same time predicting  the evolution of those features over time, an aspect that builds anticipations and allows creation of surprise, validation or violation of expectation and building of tensions and resolutions in a musical narrative.
In order to allow quantitative approach to analysis of what's going on "in the musical mind", we propose an information theoretic model for the relation between four factors: the signal past $X$, the signal present $Y$, and their internal or mental representation in terms of latent variables $Z$, and and $T$, respectively. This highly simplified model assumes a set of Markov chain relations, as shown in Figure \ref{fig:1}, between the past of the signal $X$ that is encoded into a latent representation $Z$,  the future of the signal $Y$ that depends on its past $X$, and its approximation by decoding from a latent representation $T$ that is predicted from past latent representation $Z$. 

\begin{figure}[!htb] %[!t]
\centering
\includegraphics[width=65mm]{figure/xyzt-brain-music.png}
\caption{Graph of the model variable statistical dependencies. The letter "e" represents an encoding that will be parametrized according to different complexity through changing the bit-rate between the encoder and decoder in VAE.}\label{fig:Graph-Model}
\label{fig:1}
\end{figure}

Using the Markov relation $Z-X-Y$, we can try to formulate a mathematical expression for the goals underlying the learning process of such a musicing system \cite{Musicing}. Our expression for the optimization goal comprises of a combination of factors - simplicity of representation versus its prediction ability. Accordingly, we are looking for representation that is minimizing the discrepancy, or statistical distortion, between signal prediction using complete information about the past $X$, versus its prediction capability by using a simplified encoding of the past $Z$. The overall quality of such error is averaged over all possible encoding pairs $X,Z$ of the musical surface and its latent code, respectively.
\begin{align*}
   \langle & D_{KL}(p(Y|X)||p(Y|Z)) \rangle_{p(X,Z} = I(X,Y|Z)\\
   & = I(X,Y)-I(Z,Y)  
%    & = \int p(x_{past},z) p(x|x_{past}) \log \frac{p(x|x_{past})}{p(x|z)} dxdx_{past}dz \\
%    & = \int p(x_{past},z,x) \log \frac{p(x|x_{past})p(x_{past})}{p(x_{past})p(x)}\frac{p(x)p(z)}{p(x|z)p(z)} dx dx_{past}dz \\
%    & = = I(x_{past},x|z)
    \label{eq:PredKL}
\end{align*}
Since $I(X,Y)$ are independent of $p(Z|X)$, minimizing the error between the true conditional probability of the future on its past $p(Y|X)$, compared to probability of the future conditioned on the latent representation $P(Y|Z)$, requires minimization of $-I(Z,Y)$, or maximizing the mutual information between the encoding of the past and the signal future.  

Using similar relations, we can express $I(Z,Y) = I(Z,T)-I(Z,T|Y)$. This equation is a central part of the estimation and experimental approach described in this paper, as if combines two factors - the ability of predicting the future of the musical surface $Y$ from the latent (mental) representation that the system of the past $Z$ is expressed as the difference between predicting the next latent representation $T$ and the residual or redundant information between $Z,T$ once the next elements form the musical surface $Y$ is revealed. If we assume that the latent representation fully captures the surface, or in other words, if $T=Y$, then full knowledge about the musical surface is already contained in the imaginary or latent states sequence, resulting in zero residual information $I(Z,T|Y)=0$. In such case we may ignore the right side of the equation, which creates an exceptional situation where maximizing the predictive ability of the model is achieved by maximization of the information rate (IR) of the latent states sequence $I(Z,T)$, measured as mutual information between past and present of the sequence. In case the imaginary anticipation is not perfect, we have a non-zero surprisal factor $I(Z,T|Y)$ that can be also understood as the different between latent information rate and latent past to data (surface) future $I(Z,T|Y) = I(Z,T) - I(Z,Y)$. In other words, the fact that the imaginary past cannot fully predict the musical future is the basis for musical tension that emerges in the listening process or deliberately established during the composition phase.

\subsection{Surface Representation and Information Dynamics}
Using information theoretical approach, we need to know the probability distribution of all the variables in order to compute the appropriate information measures. Since we do not know the true probability dynamics of the musical surface that govern transitioning from past $X$ to future $Y$, $P(X,Y)$, we will substitute it by a variational approximation at the best possible quality. 
The encoding of $X$ and $Y$ into latent codes $Z$ and $T$ respectively, can be done by a Variational Auto-Encoder (VAE). It was shown that minimization of $I(X,Z)$ under distortion constraint $D(X,Z)$ is equivalent to learning a representation by minimizing of Evidence Lower Bound (ELBO)\cite{BrokenELBO}. 
Combining the prediction quality criteria  ELBO and the prediction 
This gives us the model loss that combines both latent and temporal information aspect as follows 
\begin{equation}
    \mathcal{L} = I(X,Z) + \beta \langle D(X, Z) \rangle - \gamma (I(Z,T)-I(Z,T|Y))
    \label{eq:DeepRD}
\end{equation}
It should be noted that there is a separation between the past variables $X$ and $Z$ and the future $T,Y$. In the following we will train separately a neural network to minimize the $X,Z$ part of the loss, and then manipulate $Z,T$ by lossy encoding.

In the following we will compare the dynamics of latent states at different representation qualities. For simplicity and clarity of the following discussion and experiments, we will assume that there is an equivalence between full-rate latent representation and the surface data. In other words, we will assume $X=Z_{full-rate}$ and $Y = T_{full-rate}$. In the next paragraph we will describe how we can reduce the bit-rate of the encoding, as a way of simulating a limited capacity of the mental representation. Then we will discuss how the quality of the bit-rate limited representation and its dynamics can be estimated.
%This derivation suggests a new training criteria for musical neural models that combine both latent and temporal information as 
%\begin{equation}
%    \mathcal{L} = I(x_{past},z) + \beta \langle d(x_{past}, z) \rangle - \gamma I(z,x)
%    \label{eq:DeepRD}
%\end{equation}
%The optimization of $\mathcal{L}$ promises finding a solution that simultaneously minimizes the rate between musical surface and latent state and maximizes the mutual information between the latent states and future of the musical surface, while balancing the distortion between the latent states and the reconstructed surface. 

\subsection{Bit-rate limited Encoding}
Using a noisy channel between encoder and decoder we are able to introduce complexity control over the encoding through the use of bit-allocation algorithms. It is assumed in VAE that the latent states are distributed as multi-variate uncorrelated Gaussians. The rate distortion of such signal is
\begin{equation}
    R(D) = 
    \begin{cases}
        \frac{1}{2} log_2 \frac{\sigma^2}{D}, & \text{if $0 \leq D \leq \sigma^2$}\\
        0, & \text{if $D > \sigma^2$}.
    \end{cases}
\end{equation}
This rate-distortion can be converted to distortion-rate function $D(R)=\sigma^2 2^{-2R}$, which can be efficiently achieved for a multivariate Gaussian channel by = so called reverse water filling algorithm that starts with a predefined bit-regime and successively allocates one bit at a time to the strongest component, every time reducing the component variance by factor of four and repeating the process until all bits in the bit-pool are exhausted. One should note that channels with variance less then allowed distortion, or channels that run out of bits for a given rate, are given zero bits and thus are eliminated from the transmission.
We use such channel to reduce the rate of the decoder by adding noise or eliminating some of the weaker latent components. 

Schematic representation of the channel inclusion in the auto-encoder architecture is given by Figure \ref{fig:AE_noisy_channel}.
\begin{figure}
    \centering
%    \includegraphics[width=\linewidth]
    \includegraphics[width=4cm, height=6cm]{figure/VAE_with_NoisyChannel.png}
     \caption{Noisy channel between encoder and decoder}
    \label{fig:AE_noisy_channel}
\end{figure}
Performing finite bit-size encoding and transmission of the binary quantized latent values from encoder $Z_e$ to decoder $Z_d$ is not required, since we are interested in gating and biasing the original signal towards the prior distribution by encoding it at limited bitrate, which is given by the following optimal channel \cite{Berger}
\begin{align}
     Q(z_d|z_e) & = Normal(\mu_d,\sigma_d^2) \\
    \mu_d & = z_e + 2^{-2R}(\mu_e - z_e) \\
    \sigma^2_d & = 2^{-4R}(2^{2R}-1)\sigma^2_e
\end{align}

The practical way of using this channel in our bit-rate controlled model is by plugging each latent encoder value, mean and variance into the above equation, giving us the mean and variance of the decoder's conditional probability, and then picking at random the decoder value according to this distribution. One can see that channels with zero rate will transmit deterministic  mean value of that element, while channels with infinite rate will transmit the encoder values unaltered. 

\subsection{Estimation of Information Dynamics using VMO}
Variable Markov Oracle (VMO) is an generative machine learning method based on the Factor Oracle (FO) string matching algorithm. The VMO suffix tree data structure allows for various media-data generation \cite{Wang2014}. In order to operate on complex multivariate time series data, \emph{VMO} quantizes a signal $x_1^T = x_1,x_2,\dots, x_t, \dots, x_T$, into a symbolic sequence $s_1^T = s_1,s_2,\dots,s_t,\dots,s_T$, over a finite alphabet $s \in S$ Relating this to the deep information dynamics model, we denote as $X=x_{past}=x_1^{T-1}$ and $Y=x_{present}=x_T$. 
The computation of Information Dynamics is done using the Information Rate (IR) measure $I(X,Y$ of mutual information between past and present of the musical signal. Equivalently, it applied to latent states representation, to estimate $I(Z,T)$. Once the symbolization process in VMO is applied to a time series, IR can be estimated by applying a string compression method $C$, using the approximation $I(X,Y) = H(Y)-H(Y|X) \approx C(Y) - C(Y|X)$, where we substitute entropy $H$ with compression $C$, with $C(Y) = log2(|S|$ being individual symbol over alphabet $S$, and $C(Y|X)$ is a block-wise encoding that recursively points to repeated sub-sequences, such as in the Lempel-Ziv or Compror string compression algorithms \cite{Wang2015}.
The essential step for symbolization in \emph{VMO} is finding a threshold value, $\theta$ that partitions the time-series data values into discrete categories. The threshold $\theta$ is used to determine if the incoming $x_t$ is similar to one of the frames following the suffix link started at $t-1$. \emph{VMO} assigns two frames, $x_i$ and $x_j$, the same label $s_i=s_j \in \Sigma$ if $||x_i-x_j||\le\theta$. 
In \cite{VMO} Variable Markov Oracle (VMO) was proposed as an efficient method for estimating IR. 
At each bit-rate we apply VMO analysis to estimate the information dynamics of that representation. This gives us an estimation of $I(Z,T)$
at different bit-rates, as discussed in the experimental section. 
Alternative approaches to estimation of predictive information are also possible, such as using RNN models. We use VMO since it is able to capture much longer time dependencies then regular RNN's. Exploring long memory models such as attention RNNs or transformers will be considered in a future research.

\subsection{Estimation of the Predictive Encoding Quality}
In order to estimate the quality of the encoding, we need to estimate the information between past embedded representation $Z$ and the future musical surface data $Y$, $I(Z,Y)$. In the first encoding step we already minimized a related quality $I(X,Z)$ (and $I(Y,T)$ as well), but training a VAE. This process of learning the latent codes was done based on optimization of instantaneous representation quality, which we assumed fixed at this stage. This gives us two different random variables $Z$ and $Y$, which will be for any practical purposes replaced in the experiments with $Y = Z_{full-rate}$, and $Z = Z_{limited-rate}$. Both of these variables are available to us after the two steps of initial VAE encoding and bit-rate compression are completed.
We use MINE (Mutual Information Neural Estimation) \cite{MINE} as a method for estimating $I(Z,Y)$ (or in practice $I(Z_{full-rate}, Z_{limited-rate}$). The network used in the experiments comprises of two parallel networks with shared weights, one receiving ordered pairs of $Z,Y$ and the other receiving a pair of $Z$ with a shuffled version of $Y$, both mapped though two fully connected layers with 30 hidden states with a dropout layer of $0.3$ and eventually mapped to a single output. The two networks are combined into one loss function according to the MINE estimation algorithm, with the networks serving as it's mapping function. The training was done until approximate convergence, as shown in the results section. 
%The choice of the mapping function parameter was done by trail and error, to assure that the algorithm converges. 

\begin{figure}[!htb] %[!t]
    \includegraphics[width=\columnwidth]{figure/PredictiveCoding.png}
    \caption{Estimation of the predictive quality of bit-limited representation. Sub-figures A,B,C show the bit-rate allocation at rates 10, 50, and 10000, respectively. The x-axis corresponds to the 500 latent state variables, with portions showing no-bit allocation basically not being transmitted or accounted for in the latent representation. Sub-figures D,E,F show the MINE estimate as function of the training epochs, for these rates.}
    \label{fig:3}
\end{figure}

\subsection{Suprisal and Information measures}
In the section on Deep Information Dynamics we introduced the concept of surprisal $I(Z,T|Y) = I(Z,T) - I(Z,Y)$, defined as the difference between IR of the latent sequence and the predictive quality of the musical surface from previous latent states. It should be noted that from pure mathematical definitions perspective, both factors require averaging over the complete data, resulting in a summary statistic that is time independent. In our application of VMO, an instantaneous information rate can be obtained by considering the compression rate at each point in time along the sequence: locations of long repeated factors are encoded more efficiently (thus having lower IR), while data points that are novel are encoded either individually or in shorter block, thus having a less compression difference compared to individual symbol encoding. 

In contrast to VMO, the MINE method averages over the whole set of data points in $Z$ and $Y$, thus providing a single number. Accordingly, the surprisal, as considered in the experimental section, comprises of the time varying IR profile with a constant penalty factor of predictive encoding prediction quality subtracted from it. Since VMO and MINE are based on very different algorithms, the units of IR and encoding MINE estimates are not compatible, so we analyze them separately. 

\section{Experimental Results}
In order to demonstrate the utility of the proposed model for music analysis, we show below the results of deep information rate analysis of an single musical piece. The purpose of the experiments is to explore the relation between complexity of the encoding and its time predictive properties, considering in terms of changes occurring in the musical materials over time, as well as different levels of musical complexity that are captured by each bit-rate limited representation.

In the first step of the experiment, we trained a VAE on set of MIDI files from LABROSA\cite{LABROSA} training set, containing piano performances in the classical music genre. Our VAE model had an input layer that corresponded to one bar (16 steps) of polyphonic music. The input encoding was done as multi-hot representation, with note numbers (pitches) and duration captured into a single vector\footnote{We used midiToNoteStateMatrix encoding from \url{https://www.kaggle.com/chetanmj23/pop-music-collection?select=midi_manipulation.py}}.
The VAE had a single hidden layer of size 500. The trained weights of the VAE encoder were saved for later use, and the encoder part of VAE was used to create the representation for the next step of music analysis.

In the second step of the experiment we used a different MIDI files, taken from the LABROSA test set. In the example below we use a MIDI file of the Prelude and Fugue No. 2 in C Minor, BWV 847, by J.S.Bach. The bit-allocation algorithm was used to reduce the representation complexity of VAE encodings, and VMO was used to compute the optimal symbolization by exhaustive search over possible threshold values and estimating the Information Rate of the sequence in terms of the compression gain achieved by FO-based string compression measure. MINE was used to compute the Mutual information between the bit-rate limited encoding of a previous bar and a full-rate encoding of the current bar, averaged on the whole piece. 

Figure \ref{fig:2} shows the Information Rate of the latent representation $I(Z,T)$ at different bit-rates. As a point of reference we provide harmonic and thematic analysis of the piece\footnote{\url{http://bachwelltemperedclavier.org/pf-c-minor.html}} in sub-figure B, and the score rendering in sub-figure C. 
Figure \ref{fig:3} shows the predictive quality of latent representation one frame into the future $I(Z,Y)$ (We remind that $Y$ is estimates as $Z_{full-rate})$. The bit-allocation to the 500 latent states is shown at the top of the in Figure, and the estimated Mutual Information at each encoding rate is shown below.
Information Rate). 

\begin{figure}[!htb] %[!t]
    \includegraphics[width=\columnwidth]{figure/IR_Results.png}
    \caption{Analysis of Information Rate using VMO at A:full-rate, C: rate 50, D: rate 10. Sub-figure B shows harmonic analysis of the Prelude and Thematic analysis of the Fugue, Sub-figure C shows the full score.}
    \label{fig:2}
\end{figure}

It is evident that changing the representation quality by lowering the bit-rate has dramatic effect on the information dynamics of the latent representation. If we consider such information dynamics as expectations formed by our imagination, the points where the expectations differ at different bit-rates are assumed to carry creative or experiential significance. For instance, even in this rough analysis one can see that the major events, such as transition to new materials in bars 25-27 cause a drop in Information Rate. Also the development of thematic material in the Figure starting around bars 44-45 causes increase in Information Rate in both full rate and rate of 50\footnote{The units of bit-rate reduction are total bits per measure}. For high bit-rates the graph of IR seems to be relatively robust, and for very low-rates the quality of musical reconstruction seems to be too low to capture significant musical information. For rate of 10 we see that after a short initial period where materials were not repetitive (low Information rate), the rest of the music is perceived as one long repetition (high IR). 

To account for surprisal, the IR graphs have to take into account also the penalty factor of the predictive encoding quality. As mentioned above, such fixed penalty is not indicative of instantaneous changes in predictive quality of the musical surface from the latent representation. The results of MINE analysis show, As expected, that at low bit-rate encoding, the quality of prediction is lower, thus affecting less the overall surprisal relative to changes in IR, while in high bit-rate such penalty is more significant. Despite the fact that MINE algorithm trains a neural network to capture the joint versus independent statistics of $Z,Y$ pairs, that neural network cannot be used to make actual predictions. In future work we plan to train a predictor in order to compute an instantaneous error, so that both factors in surprisal could be combined or considered in parallel as functions of time.

\section{Summary}
In this paper we presented a work in progress for developing a theoretical framework of musical surprisal, formulated in terms of information theoretical relations between full-rate (high-fidelity) encoding of the musical data, and a lower complexity latent encoding that models mental or imaginary musical representations. The motivation for this type of modeling comes from the cognitive idea that musical creativity and musical perception obey a trade-off between abstraction or simplified representation of music that captures more salient or structural aspects of music, and perceptual sensibility to the musical surface that is abundant in detail. To the best of our knowledge, no such conceptual or computational framework had been previously offered. The results presented in the paper are meant to demonstrate the analytical potential of such approach, outlining also the algorithmic tools used at each step. Further research and detailed analysis of richer repertoire will be presented in supplemental materials. 




%---



==> paper_contents_short.tex <==
\section{Introduction}
Music Information Dynamics is a field in music analysis that is inspired by theories of musical anticipation \cite{meyer56emotion}\cite{huron06sweet}, which deals with quantifying the amount of information passing over time between past and future in musical signal \cite{dubnov06spectral},\cite{Abdallah}. Music Information Dynamics can be estimated in terms of Information Rate, which is defined as mutual information between past and future of a musical signal. Generative models that maximize Information rate were shown to provide good results in machine improvisation systems %cite{Assayag2004},
\cite{pasquier2017introduction}. 
In this paper we introduce the concept of deep musical information dynamics analysis that offers a combined approach to learning representation and predictive information, considering the trade off between encoding complexity of short-term musical structures and maximizing the information rate from past into future. 

%------

\subsection{Deep Information Dynamics}
We investigate music by analyzing the relation between information in the signal past $X$ and present $Y$, represented by latent variables $Z$, and $T$, respectively. This establishes a circular Markov chain shown in Figure \ref{fig:Graph-Model}, with "e" label representing the encoding operation, as explained below.

\begin{figure}[!htb] %[!t]
\centering
\includegraphics[width=35mm]{figure/xyzt.png}
\caption{Graph of the model variable statistical dependencies}\label{fig:Graph-Model}
\end{figure}

Using the Markov relation $Z-X-Y$, we write the prediction goal in terms of minimizing a discrepancy between signal prediction from complete information $X$, and prediction from an encoding $Z$, averaged over all possible encoding pairs $X,Z$ 
\begin{equation}
   \langle & D_{KL}(p(Y|X)||p(Y|Z)) \rangle_{p(X,Z)} = I(X,Y|Z)\\
   & = I(X,Y)-I(Z,Y)  
%    & = \int p(x_{past},z) p(x|x_{past}) \log \frac{p(x|x_{past})}{p(x|z)} dxdx_{past}dz \\
%    & = \int p(x_{past},z,x) \log \frac{p(x|x_{past})p(x_{past})}{p(x_{past})p(x)}\frac{p(x)p(z)}{p(x|z)p(z)} dx dx_{past}dz \\
%    & = = I(x_{past},x|z)
    \label{eq:PredKL}
\end{equation}

Since $I(X,Y)$ are independent of $p(Z|X)$, minimizing the error between the true conditional probability of the future on its past $p(Y|X)$, compared to probability of the future conditioned on the latent representation $P(Y|Z)$, requires minimization of $-I(Z,Y)$, or maximizing the mutual information between the encoding of the past and the signal future. 

Using similar relations, we write $I(Z,Y) = I(Z,T)-I(Z,T|Y)$. Ignoring the right side of the equation, we see that maximizing the predictive ability of the model is done by maximization of $I(Z,T)$. The encoding of $X$ and $Y$ into latent codes $Z$ and $T$, respectively, is done by a Variational Auto-Encoder (VAE). In \cite{BrokenELBO} it was shown that minimization of $I(X,Z)$ under distortion constraint $D(X,Z)$ is equivalent to VAE learning by minimizing the negative Evidence Lower Bound (NegELBO).
Combining NegELBO as representation quality criteria with  prediction distortion term, gives the total model loss that combines both latent and temporal information: 
\begin{equation}
    \mathcal{L} = I(X,Z) + \beta \langle D(X, Z) \rangle - \gamma I(Z,T)
    \label{eq:DeepRD}
\end{equation}

%This derivation suggests a new training criteria for musical neural models that combine both latent and temporal information as 
%\begin{equation}
%    \mathcal{L} = I(x_{past},z) + \beta \langle d(x_{past}, z) \rangle - \gamma I(z,x)
%    \label{eq:DeepRD}
%\end{equation}
%The optimization of $\mathcal{L}$ promises finding a solution that simultaneously minimizes the rate between musical surface and latent state and maximizes the mutual information between the latent states and future of the musical surface, while balancing the distortion between the latent states and the reconstructed surface. 

\subsection{Bit-rate limited Encoding}
Using a noisy channel between encoder and decoder we are able to reduce the encoding complexity by using bit-allocation algorithm. It is assumed in VAE that the latent states are distributed as multi-variate uncorrelated Gaussians. The rate distortion of such signal is
\begin{equation}
    R(D) = 
    \begin{cases}
        \frac{1}{2} log_2 \frac{\sigma^2}{D}, & \text{if $0 \leq D \leq \sigma^2$}\\
        0, & \text{if $D > \sigma^2$}.
    \end{cases}
\end{equation}
This rate-distortion can be converted to distortion-rate function $D(R)=\sigma^2 2^{-2R}$, which can be efficiently achieved for a multivariate Gaussian channel by the so called reverse water filling algorithm. The actual encoding at limited bit-rate is given by \cite{Berger}
\begin{align}
     Q(z_d|z_e) & = Normal(\mu_d,\sigma_d^2) \\
    \mu_d & = z_e + 2^{-2R}(\mu_e - z_e) \\
    \sigma^2_d & = 2^{-4R}(2^{2R}-1)\sigma^2_e
\end{align}

\subsection{Information Rate}
Variable Markov Oracle (VMO) is an generative machine learning method based on Factor Oracle (FO) string matching algorithm. The VMO suffix tree data structure can be used for media-data generation. %\cite{Wang2014a}. 
VMO quantizes a signal $X = x_1,x_2,\dots, x_t, \dots, x_T$, into a symbolic sequence $S = s_1,s_2,\dots,s_t,\dots,s_T$ by finding a threshold value $\theta$ that partitions the feature space into discrete categories. The threshold $\theta$ is used to determine if the incoming $x_t$ is similar to one of the frames following a chain of suffix links that were previously computed for $t-1$. The new frame will be assigned same label as a frame $x_j$ consequent on the suffix link,  i.e. $s_t \leftarrow s_j$ if $||x_t-x_j||\le\theta$ \cite{VMO}. Information rate is estimated in terms of compression gain by using a FO-based string compression, effectively replacing entropy estimate by compression algorithm.

\section{Experimental Results}
In the experiment we explored the relation between complexity of the encoding and its time predictive properties. We used a set of MIDI files from LABROSA\footnote{https://labrosa.ee.columbia.edu/projects/piano/} to train a VAE encoder on short musical frames, half bar (8 steps) or whole bar (16 steps) long. The training set was used to learn several VAE models with different numbers of hidden layers. Then a different set of MIDI files taken from the test set, were encoded using the pre-trained VAE. The bit-allocation algorithm was used to reduce the representation complexity of VAE encodings, and the VMO algorithm was used to find the ideal threshold for symbolization that maximizes IR in terms of compression gain achieved for that symbolic sequence.

Our finding shows that increase in the frame encoding bit-rate results in reduction of the predictability of the signal. This is understandable since increasing the amount of detail in the representation of the sequence make it harder to find long repetitions. Interestingly enough, the symbolization threshold that is needed for optimal symbolization increases with bit-rate, evidently looking to simplify the model by performing more coarse quantization. Despite this threshold increase for higher bit-rate , we can see that the overall trend is reduction in predictive information. We have observed in many cases a secondary increase in information rate at relatively low rates. This seems to suggest that some structure was found for relatively coarse representation at a moderate threshold level. %As bitrate increases, the complexity of encoding becomes prohibitive, and VMO increases it threshold further, basically erasing the effect of fine detail in the encoding in attempt to find repetitions in a coarse symbolic representation.

\begin{figure}[!htb] %[!t]
%\centering
\minipage{0.16\textwidth}
    \includegraphics[width=\columnwidth]{figure/IRt16h1000.png}
    \par{A}
\endminipage\hfill
\minipage{0.16\textwidth}
    \includegraphics[width=\columnwidth]{figure/IRt16h500.png}
    \par{B}
\endminipage\hfill
\minipage{0.16\textwidth}
    \includegraphics[width=\columnwidth]{figure/IRt8h500.png}
    \par{C}
\endminipage
\end{figure}

\begin{figure}[!htb] %[!t]
%\centering
\minipage{0.16\textwidth}
    \includegraphics[width=\columnwidth]{figure/ITt16h1000.png}
\endminipage\hfill
\minipage{0.16\textwidth}
    \includegraphics[width=\columnwidth]{figure/ITt16h500.png}
\endminipage\hfill
\minipage{0.16\textwidth}
    \includegraphics[width=\columnwidth]{figure/ITt8h500.png}
\endminipage
\caption{Top: Information Rate as a function of representation bit-rate for two different frame sizes (16 time steps A and B, 32 time steps C) and two different encoding sizes (500 hiddent state A, 3000 hidden states B and C). Bottom: Ideal Threshold calculated by VMO for different bit-rates.} 
%Parameters are the same as in the Figure \ref{fig:IR-Bit}}\label{fig:IT-Bit}
\end{figure}

\subsection{Relation to Information Bottleneck}
The equation we reached in the previous paragraph coincides with another postulate known as Information Bottleneck (IB). This optimal criteria formulates the goal of information processing as finding a representation $Z$ carrying maximal information about target variables $Y$ while at the same time maximally compressing the source variable $X$. 
\begin{equation}
    p_{IB} (Z | X) = \max_{p(Z | X)} (I(Y,Z) - \lambda I(Z, X))
\end{equation}
This criteria is simply the negative of the probabilistic rate-distortion function we derived in the previous paragraph. Moreover, we have generalized IB to prediction-representation problem, showing the relation between latent representation complexity and its predictability.



%---



==> vertical_IR.tex <==
\subsection{Controlling "Vertical" Information Rate between Encoder and Decoder}
Using a noisy channel between encoder and decoder we are able to introduce information rate control through use of bit-allocation. It is assumed in VAE that the latent states are distributed as multi-variate uncorrelated Gaussians. The rate distortion of such signal is
\begin{equation}
    R(D) = 
    \begin{cases}
        \frac{1}{2} log_2 \frac{\sigma^2}{D}, & \text{if $0 \leq D \leq \sigma^2$}\\
        0, & \text{if $D > \sigma^2$}.
    \end{cases}
\end{equation}
This rate-distortion can be converted to distortion-rate function $D(R)=\sigma^2 2^{-2R}$, which can be efficiently achieved for a multivariate Gaussian channel by = so called reverse water filling algorithm that starts with a predefined bit-regime and successively allocates one bit at a time to the strongest component, every time reducing the component variance by factor of four and repeating the process until all bits in the bit-pool are exhausted. One should note that channels with variance less then allowed distortion, or channels that run out of bits for a given rate, are given zero bits and thus are eliminated from the transmission.
We use such channel to reduce the rate of the decoder by adding noise or eliminating some of the weaker latent components. 
%Schematic representation of the channel inclusion in the auto-encoder architecture is given by Figure %\ref{fig:AE_noisy_channel}
%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]
%% \includegraphics[width=8cm, height=2cm]
%    {images/Picture3.png}
%    \caption{Noisy channel between encoder and decoder}
%    \label{fig:AE_noisy_channel}
%\end{figure}
Performing finite bit-size encoding and transmission of the binary quantized latent values from encoder $Z_e$ to decoder $Z_d$ is not required, since we are interested in gating and biasing the original signal towards the prior distribution by encoding it at limited bitrate, which is given by the following optimal channel \cite{Berger}
\begin{align}
     Q(z_d|z_e) & = Normal(\mu_d,\sigma_d^2) \\
    \mu_d & = z_e + 2^{-2R}(\mu_e - z_e) \\
    \sigma^2_d & = 2^{-4R}(2^{2R}-1)\sigma^2_e
\end{align}

The practical way of using this channel in our bit-rate controlled model is by plugging each latent encoder value, mean and variance into the above equation, giving us the mean and variance of the decoder's conditional probability, and then picking at random the decoder value according to this distribution. One can see that channels with zero rate will transmit deterministically the mean value of that element, while channels with infinite rate will transmit the encoder values unaltered. 

%The practical way of using this channel in our bit-rate controlled model is by plugging the latent value received from the encoder into the above equation assuming zero mean and unit variance according to the prior distribution\footnote{We assume that the channel was design according to the prior}, and then choosing a random value from a normal distribution with the decoder mean and variance values to be the value passed through the channel to the decoder. One can see that components allocated zero rate will transmit deterministically the mean value of zero, while channels with infinite rate will transmit the encoder values unaltered. The limited rate components will have their mean pushed towards zero and have a small jitter added to according to channel variance at that rate.

\subsection{"Horizontal" Information Rate in Time}

Information rate of signal quantifies the information passing over time between the current measurement $Y$ and it's past $X$, formally defined in terms of the mutual information
\begin{equation}
    IR=I(Y,X) = H(Y)-H(Y|X)
\end{equation}
Maximal value of IR is obtained for signals that look instantaneously complex, thus having a high entropy $H(Y)$, but that are predictable or have little uncertainty when the signal past is taken into account, thus having low $H(Y|X)$.  In earlier studies of music information dynamics, VMO algorithm was applied to sequences of human engineered musical features. VMO is an extension of a string matching algorithm to find approximate repeated suffixes over a metric space. These suffixes are used to encode repeating blocks of the signal resulting in compression gain that is used as an estimate of the signal IR. Since the ability to find repeated suffixes depends on the level of similarity, an exhaustive search is done over all possible similarity threshold values to select the highest level of IR.
VMO has been used for comparative analysis of generative models, comparing their IR statistics to those of the original corpus. Moreover, several additional tools that are available in the VMO package allow deeper insight in the structures of music (both generative and human), such as detection and visualization of motif structure, analyzing the level of musical detail through IR graphs as function of similarity threshold, or observing the dynamics of IR over the course of a musical composition by analysis of the instantaneous repetition and predictability. It is the first time, to the best of our knowledge, that IR is being applied to analysis of the dynamic of latent states, as described next.

\section{Deep Music Information Dynamics}
 
In this work we combine the temporal and latent information rate using rate-distortion as follows. Instead of finding the most efficient or the lowest rate latent states up to a specified distortion, we are considering the lowest rate latent state representation that gives the best predictability into the future. We rewrite the rate-distortion objective using statistical similarity $D_{KL}(p(Y|X)||p(Y|Z))$ as our new distortion measure. This measure prefers latent states $Z$ that carry same information, or share the same belief about the future $Y$ as does the past $X$. Since $Z$ is an encoding derived from $X$, knowledge of $X$ supersedes that of $Z$ resulting in the following relations $p(Y|X,Z) = p(Y|Z)$, which establishes $Z-X-Y$ Markov chain relation between these three variables. Averaging over all possible $X,Z$ pairs we get 
\begin{align}
   \langle & D_{KL}(p(y|x)||p(y|z)) \rangle_{p(x,z)} \\
    & = \int p(x,z) p(y|x) log \frac{p(y|x)}{p(y|z)} dxdydz \\
    & = \int p(x,z,y) log \frac{p(y|x)p(x)}{p(x)p(y)}\frac{p(y)p(z)}{p(y|z)p(z)} dxdydz \\
    & = I[X,Y]-I[Z,Y] = I[X,Y|Z]
\end{align}
So what we have here is a probabilistic version of rate-distortion in time-belief space written as minimization problems of 
\begin{equation}
    \mathcal{L}=I(X,Z)+\beta I(X,Y|Z) = I(X,Z) - \beta I(Z,Y),
\end{equation}
where $I(X,Y)$ is neglected as it is independent of $p(Z|X)$.


\section{Composition with VAE}
As mentioned in the beginning, one of the motivations for investigating the relations between feature complexity and predictability is to use these parameters as guiding criteria for composition with generative models. VMO had been used previously as a generative model, where the suffix link relations between instances of music over time were used to remix or recombine copies of music through a cut and paste or concatenative method. The reason VMO was not used to synthesize music from scratch but rather recombine existing musical segments of variable length was that the repetition structures discovered by VMO were based on analysis of lossy features or partial representation of midi or audio that could not be reverted back to the full signal. On the other hand, deep learning model, even it they manage to compress the data significantly, they are still capable of generating an output distribution. This offer more compact and seemingly more creative approach to music generation from machine learning models, since it does not rely on storage and retrieval / recombination of literal segments from the training corpus. Having considered the advantage of generative models, there still is a significant difficulty in learning long terms structure using VAE and even using recurrent models such as RNN or LSTM.
For most practical music generation applications, neural network models are trained on a relatively short term musical segments, and when longer compositions are desired, these models are left running for longer times then they are normally designed, either by feeding back the states in a RNN manner, or retriggering random states in VAE. Finding longer term structure is possible with VMO, so one possibility is combining VMO recombination properties with NN generative properties to achieve more versatile and at the same time longer term structured generation. 
From our experience, such combination is not easy to create. One of the main reasons is the 
\section{Experimental Results}

The experiments conducted using our model comprise of querying a pre-trained model with a midi input and reducing the information available to the decoder in a controlled way by passing the encoding through a bit-rate limited channel. Then the decoded music is evaluated both qualitatively for apparent musical structure, and quantitatively in terms of its predictability by analyzing the temporal information rate of the latent states across different time frames. The different experiments that we conducted include:
\begin{itemize}
    \item Training a VAE and then generating new compositions by random sampling of latent states
    \item Creating an output sequence by querying the model with another midi file. 
    \item Reconstruction of a midi input query at different decoder rates by passing the latent states through a  noisy channel before decoding
\end{itemize}



\section{Summary and Discussion}
In this paper we explore several theoretical relations between "vertical" information rate between musical surface and latent states that are learned by a variational auto-encoder, and the predictability of sequence of these latent states over time as a "horizontal" information rate. We conducted several experiments where we deliberately reduced the quality of the decoder output by adding a noisy channel between the encoder and the decoder. By doing so we were able to move from more to less meaningful latent space representations by encoding an input signal using a pre-trained encoder and degrading it in a controlled manner using bit-rate reduction before passing it to the decoder. 

It is important to note that unlike the $\beta$VAE and InfoVAE approaches that control the information rate between latent states and input data for training purposes, our study focused on pre-trained VAE with rate control of the decoding process. This allows us to use bit-rate controlled latent representations as a way to control their predictability over time. 

\section{Composition with VAE}
As mentioned in the beginning, one of the motivations for investigating the relations between feature complexity and predictability is to use these parameters as guiding criteria for composition with generative models. VMO had been used previously as a generative model, where the suffix link relations between instances of music over time were used to remix or recombine copies of music through a cut and paste or concatenative method. The reason VMO was not used to synthesize music from scratch but rather recombine existing musical segments of variable length was that the repetition structures discovered by VMO were based on analysis of lossy features or partial representation of midi or audio that could not be reverted back to the full signal. On the other hand, deep learning model, even it they manage to compress the data significantly, they are still capable of generating an output distribution. This offers more compact and seemingly more creative approach to music generation using machine learning models, since it does not rely on storage and retrieval / recombination of literal segments from the training corpus. Having considered the advantage of generative models, there still is a significant difficulty in learning long terms structure using VAE and even using recurrent models such as RNN or LSTM.
For most practical music generation applications, neural network models are trained on a relatively short term musical segments, and when longer compositions are desired, these models are left running for longer times then they are normally designed, either by feeding back the states in a RNN manner, or retriggering random states in VAE. Finding longer term structure is possible with VMO, so one possibility is combining VMO recombination properties with NN generative properties to achieve more versatile and at the same time longer term structured generation. From our experience, such combination is not easy to create. One of the main reasons is the 

\subsection{Future research}

In order to analyze the temporal performance of generative models, we consider how the internal working of the learning model affect the ability , which in our case is based on variational auto-encoding deep learning that represents the musical data in terms of a latent state $Z$. In this model, the listener, or the generator that learned the musical model by listening to music from a corpus, Considering this model in terms of information transfer over time, we see that when the past is known, the probability of the future does not depend on the latent state $z$, $Prob(x | \overleftarrow{x},z) = Prob(x | \overleftarrow{x})$
%$prob(future | past, current latent state) = prob(future | past)$. 
Conversely, the latent state does capture some of the information passing from the past to the future, so in our investigation we would like to asses the difference between having a full knowledge of the past, which is assumed to be available in the original formulation of IR, and the information flow through the generative model (also sometimes also called information transfer [Schreiber]) that is measured as information transfer through a bottleneck of the latent state. 
In other words, we assume that both the composer / music generator and the listener share a latent representation z, in the following way: past musical data are encoded into latent representation, and the encoding that we desire is one in which the information into the future is maximized. Writing out the optimization problem in mathematical terms becomes a problem of measuring the loss one encounters in replacing the past with the latent encoding $z$ [Still], which can be measured by
$D_{KL}[p(x | \overleftarrow{x}) ||  p(x | z)]$ 
%KL Distance[prob(future | past) || prob(future | latent encoding)]


